PLD: A Choice-Theoretic List-Wise Knowledge Distillation

Knowledge distillation is a model compression technique in which a compact "student" network is trained to replicate the predictive behavior of a larger "teacher" network. In logit-based knowledge distillation, it has become the de facto approach to augment cross-entropy with a distillation term. Typically, this term is either a KL divergence that matches marginal probabilities or a correlation-based loss that captures intra- and inter-class relationships. In every case, it acts as an additional term to cross-entropy. This term has its own weight, which must be carefully tuned. In this paper, we adopt a choice-theoretic perspective and recast knowledge distillation under the Plackett-Luce model by interpreting teacher logits as "worth" scores. We introduce "Plackett-Luce Distillation (PLD)", a weighted list-wise ranking loss. In PLD, the teacher model transfers knowledge of its full ranking of classes, weighting each ranked choice by its own confidence. PLD directly optimizes a single "teacher-optimal" ranking. The true label is placed first, followed by the remaining classes in descending teacher confidence. This process yields a convex and translation-invariant surrogate that subsumes weighted cross-entropy. Empirically, across CIFAR-100, ImageNet-1K, and MS-COCO, PLD achieves consistent gains across diverse architectures and distillation objectives, including divergence-based, correlation-based, and feature-based methods, in both homogeneous and heterogeneous teacher-student pairs.

==> sections/tables/N_students.tex <==
% \begin{table}[ht]
% \centering
% \small
% \caption{Distillation performance across student–teacher pairs on ImageNet-1K. Top-1/Top-5 accuracy (\%) for the teacher, KD, DIST, and PLD. \(\Delta_{\mathrm{DIST}}\) and \(\Delta_{\mathrm{KD}}\) denote the Top-1 improvement of PLD over DIST and KD, respectively.}
% \label{tab:arch-generalization}
% \begin{tabular}{ll|cc|cc|cc|cc|cc}
% \toprule
% Student & Teacher 
%  & \multicolumn{2}{c|}{Teacher} 
%  & \multicolumn{2}{c|}{KD} 
%  & \multicolumn{2}{c|}{DIST} 
%  & \multicolumn{2}{c|}{PLD} 
%  & \(\Delta_{\mathrm{DIST}}\) 
%  & \(\Delta_{\mathrm{KD}}\) \\
% \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
%  & & Top1 & Top5 & Top1 & Top5 & Top1 & Top5 & Top1 & Top5 & Top1 & Top1 \\
% \midrule
% vit-s
%  & vit-l
%  & 85.85 & 97.83
%  & 75.33 & 91.71
%  & 74.91 & 91.94
%  & 75.63 & 92.32
%  & 0.72 & 0.30 \\
% resnet50
%  & resnet152
%  & 82.82 & 96.12
%  & 76.80 & 93.16
%  & 76.60 & 93.30
%  & 77.30 & 93.28
%  & 0.70 & 0.50 \\
% mobilenetv4-m(conv)
%  & mobilenetv-l(conv)
%  & 84.67 & 97.11
%  & 74.86 & 92.03
%  & 75.40 & 92.42
%  & 75.72 & 91.83
%  & 0.32 & 0.86 \\
% mobilenetv4-m(conv)
%  & mobilenetv-l(conv)
%  & 84.67 & 97.11
%  & 67.38 & 88.01
%  & 70.05 & 88.91
%  & 70.06 & 88.42
%  & 0.02 & 2.68 \\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[ht]
% \centering
% \small
% \caption{Top-1 accuracy (\%) for distillation across student–teacher architectures on ImageNet-1K. \(\Delta_{\mathrm{DIST}}\) and \(\Delta_{\mathrm{KD}}\) denote PLD’s Top-1 gain over DIST and KD, respectively.}
% \label{tab:arch-generalization}
% \begin{tabular}{ll|cccccc}
% \toprule
% \multicolumn{2}{c|}{} & \multicolumn{6}{c}{Top-1 \% Accuracy} \\
% \cmidrule(lr){3-8}
% Student        & Teacher         & Teacher & KD    & DIST  & PLD   & \(\Delta_{\mathrm{DIST}}\) & \(\Delta_{\mathrm{KD}}\) \\
% \midrule
% \multicolumn{8}{l}{\textbf{Vision Transformers}} \\
% ViT-Small      & ViT-Large       & 85.85   & 75.33 & 74.91 & \textbf{75.63} & \textbf{0.72} & \textbf{0.30} \\
% \midrule
% \multicolumn{8}{l}{\textbf{ResNets}} \\
% ResNet-50      & ResNet-152      & 82.82   & 76.80 & 76.60 & \textbf{77.30} & \textbf{0.70} & \textbf{0.50} \\
% \midrule
% \multicolumn{8}{l}{\textbf{MobileNet-v4}} \\
% Medium (conv)  & Large (conv)    & 84.67   & 74.86 & 75.40 & \textbf{75.72} & \textbf{0.32} & \textbf{0.86} \\
% Small (conv)   & Large (conv)    & 84.67   & 67.38 & 70.05 & \textbf{70.07} & \textbf{0.02} & \textbf{2.68} \\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[ht]
% \centering
% \small
% \caption{Top-1 accuracy (\%) and student model size across student–teacher pairs on ImageNet-1K.  “Teacher Acc” is the teacher’s standalone Top-1; \(\Delta_{\mathrm{DIST}}\) and \(\Delta_{\mathrm{KD}}\) are PLD’s gains over DIST and KD.}
% \label{tab:arch-generalization}
% \begin{tabular}{llc|cccccc}
% \toprule
% \multicolumn{3}{c|}{} & \multicolumn{6}{c}{Top-1 \% Accuracy} \\
% \cmidrule(lr){4-9}
% Student        & Teacher(Params)         & Params & Teacher & KD    & DIST  & PLD   & \(\Delta_{\mathrm{DIST}}\) & \(\Delta_{\mathrm{KD}}\) \\
% \midrule
% \multicolumn{9}{l}{\textbf{Vision Transformers}} \\
% ViT-Small      & ViT-Large(304.33M)       & 22.05  & 85.85   & 75.33 & 74.91 & \textbf{75.63} & \textbf{0.72} & \textbf{0.30} \\
% \midrule
% \multicolumn{9}{l}{\textbf{ResNets}} \\
% ResNet-50      & ResNet-152(60.19M)      & 25.56  & 82.82   & 76.80 & 76.60 & \textbf{77.30} & \textbf{0.70} & \textbf{0.50} \\
% \midrule
% \multicolumn{9}{l}{\textbf{MobileNet-v4}} \\
% Hybrid-Medium  & Large (conv)    & 11.07  & 84.67   & 75.47 & 75.98 & \textbf{76.33} & \textbf{0.35} & \textbf{0.86} \\
% Medium (conv)  & (32.59M)    & 9.72   &    & 74.86 & 75.40 & \textbf{75.72} & \textbf{0.32} & \textbf{0.86} \\
% Small (conv)   &    & 3.77   &   & 67.38 & 70.05 & \textbf{70.07} & \textbf{0.02} & \textbf{2.69} \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[ht]
% \centering
% \small
% \caption{Top-1 accuracy (\%) and student model size across student–teacher pairs on ImageNet-1K.  
% “Teacher Acc” is the teacher’s standalone Top-1; \(\Delta_{\mathrm{DIST}}\) and \(\Delta_{\mathrm{KD}}\) are PLD’s gains over DIST and KD.}
% \label{tab:arch-generalization}
% \begin{tabular}{llc|cccccc}
% \toprule
% \multicolumn{3}{c|}{} 
%   & \multicolumn{6}{c}{Top-1 \% Accuracy} \\
% \cmidrule(lr){4-9}
% Student         & Teacher (Params)         & Params 
%                 & Teacher & KD    & DIST  & PLD   & \(\Delta_{\mathrm{DIST}}\) & \(\Delta_{\mathrm{KD}}\) \\
% \midrule
% \multicolumn{9}{l}{\textbf{Vision Transformers}} \\
% ViT-Small       & ViT-Large\newline (304.33M)      & 22.05  
%                 & 85.85   & 75.33 & 74.91 & \textbf{75.63} & \textbf{0.72} & \textbf{0.30} \\
% \midrule
% \multicolumn{9}{l}{\textbf{ResNets}} \\
% ResNet-50       & ResNet-152 \newline(60.19M)      & 25.56  
%                 & 82.82   & 76.80 & 76.60 & \textbf{77.30} & \textbf{0.70} & \textbf{0.50} \\
% \midrule
% \multicolumn{9}{l}{\textbf{MobileNet-v4}} \\
% Hybrid-Medium (conv)
%                 & Large (conv)    & 11.07  
%                 & 84.67   & 75.47 & 75.98 & \textbf{76.33} & \textbf{0.35} & \textbf{0.86} \\
% Medium (conv)   & (32.59M)    & 9.72   
%                 & 84.67   & 74.86 & 75.40 & \textbf{75.72} & \textbf{0.32} & \textbf{0.86} \\
% Small (conv)    &    & 3.77   
%                 & 84.67   & 67.38 & 70.05 & \textbf{70.07} & \textbf{0.02} & \textbf{2.69} \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[ht]
\centering
\small
\caption{Top-1 accuracy (\%) and student model size across student–teacher pairs on ImageNet-1K.  
“Teacher Acc” is the teacher’s standalone Top-1; \(\Delta_{\mathrm{DIST}}\) and \(\Delta_{\mathrm{KD}}\) are PLD’s gains over DIST and KD.}
\label{tab:arch-generalization}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llc|cccccc}
\toprule
\multicolumn{3}{c|}{} 
  & \multicolumn{6}{c}{Top-1 \% Accuracy} \\
\cmidrule(lr){4-9}
Student            & Teacher                   & Params(M) 
                   & Teacher & KD    & DIST  & PLD   & \(\Delta_{\mathrm{DIST}}\) & \(\Delta_{\mathrm{KD}}\) \\
\midrule
% \multicolumn{9}{l}{\textbf{Vision Transformers}} \\
ViT-Small          & \shortstack{ViT-Large(304.33M)}      & 22.05  
                   & 84.80   & 75.33 & 74.91 & \textbf{75.63} & \textbf{0.72} & \textbf{0.30} \\
\midrule
% \multicolumn{9}{l}{\textbf{ResNets}} \\
ResNet-50          & \shortstack{ResNet-152(60.19M)}      & 25.56  
                   & 79.61   & 76.80 & 76.60 & \textbf{77.30} & \textbf{0.70} & \textbf{0.50} \\
\midrule
\multicolumn{9}{l}{\textbf{MobileNet-v4}} \\
Hybrid-Medium      & Large (conv)                & 11.07  
                   & 80.83   & 75.47 & 75.98 & \textbf{76.33} & \textbf{0.35} & \textbf{0.86} \\
Medium (conv)      & (32.59M)                    & 9.72   
                   & 80.83   & 74.86 & 75.40 & \textbf{75.72} & \textbf{0.32} & \textbf{0.86} \\
Small (conv)       &                             & 3.77   
                   & 80.83   & 67.38 & 70.05 & \textbf{70.07} & \textbf{0.02} & \textbf{2.69} \\
\bottomrule
\end{tabular}%
}
\end{table}

==> sections/tables/N_teachers.tex <==
% \begin{table}[t]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \caption{Top‐1 accuracy (\%) of ResNet‐50 (25.56 M) distilled from diverse teachers.  “Teacher Acc” is the teacher’s standalone Top‐1; KD, DIST, PLD, and Δ values are pending experiments.}
% \label{tab:fixed-student}
% \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l r r r r r r r}
% \toprule
% Teacher              & Params & Teacher Acc & KD & DIST & PLD & \(\Delta_{\mathrm{DIST}}\) & \(\Delta_{\mathrm{KD}}\) \\
%                      & (M)     & (\%)        &    &      &     &                           &                           \\
% \midrule

% ResNet-18            & 11.69   & 69.76       & –  & –    & –   & –       & –     \\
% ResNet-34            & 21.80   & 73.31       & –  & –    & –   & –       & –     \\
% ViT-Base/16          & 86.00   & 83.14       & –  & –    & –   & –       & –     \\
% ViT-Large/16         & 304.33  & 85.85       & –  & –    & –   & –       & –     \\
% MobileNet-v4 Large   & 32.59   & 84.67       & –  & –    & –   & –       & –     \\
% \bottomrule
% \end{tabular*}
% \end{table}

% \begin{table}[t]
% \centering
% \small
% \caption{Top‐1 accuracy (\%) of ResNet‐50 (25.56 M) distilled from diverse teachers.  “Teacher Acc” is the teacher’s standalone Top‐1; KD, DIST, PLD, and Δ values are pending experiments.}
% \label{tab:fixed-student}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{} l r r r r r r r @{}}
% \toprule
% \multicolumn{2}{c}{} 
%   & \multicolumn{6}{c}{Top-1 \% Accuracy} \\
% \cmidrule(lr){3-8}
% Teacher              & \shortstack{Params\\(M)}
%                      & \shortstack{Teacher Acc\\(\%)} 
%                      & KD   & DIST & PLD 
%                      & \(\Delta_{\mathrm{DIST}}\) 
%                      & \(\Delta_{\mathrm{KD}}\) \\
% \midrule
% ResNet-18            & 11.69   & 69.76  & – & – & – & – & – \\
% ResNet-34            & 21.80   & 73.31  & – & – & – & – & – \\
% ResNet-152           & 60.19   & 82.82  & 75.33 & 74.91 & \textbf{75.63} & \textbf{0.72} & \textbf{0.30} \\
% MobileNet-v4 Large   & 32.59   & 84.67  & – & – & – & – & – \\
% ViT-Base/16          & 86.00   & 83.14  & – & – & – & – & – \\
% ViT-Large/16         & 304.33  & 85.85  & – & – & – & – & – \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

% \begin{table}[h]
%   \renewcommand\arraystretch{1.3}
%   \setlength\tabcolsep{2mm}
%   \centering
%   \caption{\textbf{Top‐1 accuracy (\%) of ResNet-50 distilled from various teachers on ImageNet-1K.}  
%     “Params” is in millions.  $\Delta_{\mathrm{DIST}}$ and $\Delta_{\mathrm{KD}}$ show PLD’s gain over DIST and KD, respectively.}
%   \label{tab:teachers-diverse}
%   \footnotesize
%   \begin{tabular}{lrrrrrrr}
%     \toprule
%     \textbf{Teacher} & \textbf{Params} & \textbf{Teacher} & \textbf{KD} & \textbf{DIST} & \textbf{PLD}
%       & \(\boldsymbol{\Delta_{\mathrm{DIST}}}\) 
%       & \(\boldsymbol{\Delta_{\mathrm{KD}}}\) \\
%     & (M) & \textbf{Top-1} 
%       & \textbf{Top-1} 
%       & \textbf{Top-1} 
%       & \textbf{Top-1} 
%       & (PLD–DIST) & (PLD–KD) \\ 
%     \midrule
%     MobileNet-v4 Medium  
%       & 21.94 & 83.00 
%       & 76.85 & 77.00 & 77.34 
%       & \(\,+0.34\) & \(\,+0.49\) \\

%     MobileNet-v4 Large 
%       & 32.59 & 84.67 
%       & 73.98 & 75.05 & 75.53 
%       & \(\,+0.48\) & \(\,+1.55\) \\

%     ViT-Base/16                
%       & 86.00 & 83.14 
%       & 74.27 & 75.40 & 75.80 
%       & \(\,+0.40\) & \(\,+1.53\) \\

%     ViT-Large/16               
%       & 304.33 & 85.85 
%       & 75.98 & 76.86 & 77.38 
%       & \(\,+0.52\) & \(\,+1.40\) \\

%     ResNet-152                 
%       & 60.19 & 82.82 
%       & 76.80 & 76.60 & 77.30 
%       & \(\,+0.70\) & \(\,+0.50\) \\

%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}[h]
%   \renewcommand\arraystretch{1.3}
%   \setlength\tabcolsep{2mm}
%   \centering
%   \caption{\textbf{Top‐1 accuracy (\%) of ResNet-50 distilled from various teachers on ImageNet-1K.}  
%     “Params” is in millions.  $\Delta_{\mathrm{DIST}}$ and $\Delta_{\mathrm{KD}}$ show PLD’s gain over DIST and KD, respectively.}
%   \label{tab:teachers-diverse}
%   \footnotesize
%   \begin{tabular}{lrr|rrrr}
%     \toprule
%     \multicolumn{3}{c|}{} 
%       & \multicolumn{4}{c}{Top-1 \% Accuracy} \\
%     \cmidrule(lr){4-7}
%     \textbf{Teacher} 
%       & \textbf{Params} 
%       & \textbf{Teacher} 
%       & \textbf{KD}  
%       & \textbf{DIST} 
%       & \textbf{PLD}
%       & \(\boldsymbol{\Delta_{\mathrm{DIST}}}\;/\;\boldsymbol{\Delta_{\mathrm{KD}}}\) \\
%     & (M) & \textbf{Top-1} 
%       &  &  &  &  \\
%     \midrule
%     MobileNet-v4 Hybrid Medium  
%       & 21.94 & 83.00 
%       & 76.85 & 77.00 & 77.34 
%       & {\small\(+0.34\)/\(+0.49\)} \\

%     MobileNet-v4 Conv AA Large 
%       & 32.59 & 84.67 
%       & 73.98 & 75.05 & 75.53 
%       & {\small\(+0.48\)/\(+1.55\)} \\

%     ViT-Base/16                
%       & 86.00 & 83.14 
%       & 74.27 & 75.40 & 75.80 
%       & {\small\(+0.40\)/\(+1.53\)} \\

%     ViT-Large/16               
%       & 304.33 & 85.85 
%       & 75.98 & 76.86 & 77.38 
%       & {\small\(+0.52\)/\(+1.40\)} \\

%     ResNet-152                 
%       & 60.19 & 82.82 
%       & 76.80 & 76.60 & 77.30 
%       & {\small\(+0.70\)/\(+0.50\)} \\

%     \bottomrule
%   \end{tabular}
% \end{table}

% \begin{table}[h]
%   \renewcommand\arraystretch{1.3}
%   \setlength\tabcolsep{2mm}
%   \centering
%   \caption{\textbf{Top‐1 accuracy (\%) of ResNet-50 distilled from various teachers on ImageNet-1K.}  
%     “Params” is in millions.  $\Delta_{\mathrm{DIST}}$ and $\Delta_{\mathrm{KD}}$ show PLD’s gain over DIST and KD, respectively.}
%   \label{tab:teachers-diverse}
%   \footnotesize
%   \begin{tabular}{l r | r r r r | r}
%     \toprule
%     \multicolumn{2}{c|}{} 
%       & \multicolumn{4}{c|}{Top-1 \% Accuracy} 
%       & \multirow{2}{*}{\(\Delta_{\mathrm{DIST}}/\Delta_{\mathrm{KD}}\)} \\
%     \cmidrule(lr){3-6}
%     \textbf{Teacher} 
%       & \textbf{Params} 
%       & \textbf{Teacher} 
%       & \textbf{KD}  
%       & \textbf{DIST} 
%       & \textbf{PLD}
%       &  \\
%     & (M) & \textbf{Top-1} 
%       &  &  &  &  \\
%     \midrule
%     MobileNet-v4 Hybrid Medium  
%       & 21.94 & 83.00 
%       & 76.85 & 77.00 & 77.34 
%       & {\small\(+0.34\)/\(+0.49\)} \\

%     MobileNet-v4 Conv AA Large 
%       & 32.59 & 84.67 
%       & 73.98 & 75.05 & 75.53 
%       & {\small\(+0.48\)/\(+1.55\)} \\

%     ViT-Base/16                
%       & 86.00 & 83.14 
%       & 74.27 & 75.40 & 75.80 
%       & {\small\(+0.40\)/\(+1.53\)} \\

%     ViT-Large/16               
%       & 304.33 & 85.85 
%       & 75.98 & 76.86 & 77.38 
%       & {\small\(+0.52\)/\(+1.40\)} \\

%     ResNet-152                 
%       & 60.19 & 82.82 
%       & 76.80 & 76.60 & 77.30 
%       & {\small\(+0.70\)/\(+0.50\)} \\
%     \bottomrule
%   \end{tabular}
% \end{table}

\begin{table}[ht]
\centering
\small
\caption{Top-1 \% accuracy of ResNet-50 distilled from diverse teachers on ImageNet-1K.  
“Params” is the teacher’s parameter count in millions.  
\(\Delta_{\mathrm{DIST}}\) and \(\Delta_{\mathrm{KD}}\) report PLD’s gains over DIST and KD, respectively.}
\label{tab:fixed-student}
\resizebox{\columnwidth}{!}{%
  \begin{tabular}{l r | c c c c | c c}
    \toprule
    \multicolumn{2}{c|}{} 
      & \multicolumn{4}{c|}{Top-1 \% Accuracy} 
      & \multicolumn{2}{c}{\(\Delta\)} \\
    \cmidrule(lr){3-6} \cmidrule(lr){7-8}
    \textbf{Teacher} & \textbf{Params (M)}
      & \textbf{Teacher} & \textbf{KD} & \textbf{DIST} & \textbf{PLD} 
      & \(\boldsymbol{\Delta_{\mathrm{DIST}}}\) & \(\boldsymbol{\Delta_{\mathrm{KD}}}\) \\
    \midrule
    ResNet-152                 
      & 60.19 & 79.61 & 76.80 & 76.60 & \textbf{77.30}  & \textbf{0.70} & \textbf{0.50} \\
    \midrule
    MobileNet-v4 Hybrid Medium  
      & 11.07 & 78.66 & 76.85 & 77.00 & \textbf{77.34}  & \textbf{0.34} & \textbf{0.49} \\

    MobileNet-v4 Conv Large  
      & 32.59 & 80.83 & 73.98 & 75.05 & \textbf{75.53}  & \textbf{0.48} & \textbf{1.55} \\

    ViT-Base/16                
      & 86.57 & 82.07 & 74.27 & 75.40 & \textbf{75.80}  & \textbf{0.40} & \textbf{1.53} \\

    ViT-Large/16               
      & 304.33 & 84.80 & 75.98 & 76.86 & \textbf{77.38} & \textbf{0.52} & \textbf{1.40} \\


    \bottomrule
  \end{tabular}%
} % end \resizebox
\end{table}


==> sections/tables/baseline.tex <==

% \begin{table}[ht]
% \centering
% \small
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Loss $L$} & $\alpha$ & $\beta$ & $\gamma$ & $\tau$ & \textbf{Top‐1 Acc.\,\%} & \textbf{KL} \\
% \midrule
% CE                   & —    & —    & —    & —   & 71.354 & —         \\

% KD ($\tau=2$)        & 0.0  & —    & —    & 2   & 75.974 & 0.229444  \\
%                      & 0.1  & —    & —    & 2   & \textbf{76.718} & 0.280689  \\
%                      & 0.2  & —    & —    & 2   & 76.614 & 0.320531  \\
%                      & 0.3  & —    & —    & 2   & 76.388 & 0.355898  \\
%                      & 0.4  & —    & —    & 2   & 76.286 & 0.385557  \\
%                      & 0.5  & —    & —    & 2   & 76.098 & 0.432864  \\
%                      & 0.6  & —    & —    & 2   & 75.904 & 0.459411  \\
%                      & 0.7  & —    & —    & 2   & 75.798 & 0.510476  \\
%                      & 0.8  & —    & —    & 2   & 75.494 & 0.567144  \\
%                      & 0.9  & —    & —    & 2   & 74.244 & 0.688823  \\
% \midrule
% DIST ($\tau=1$)      & 1.0  & 2.0  & 2.0  & 1   & 75.618 & 0.698789  \\
%                      & 0.0  & 0.50 & 0.50 & 1   & 76.368 & 0.537605  \\
%                      & 0.1  & 0.45 & 0.45 & 1   & \textbf{76.516} & 0.626846  \\
%                      & 0.2  & 0.40 & 0.40 & 1   & —      & —         \\
%                      & 0.3  & 0.35 & 0.35 & 1   & —      & —         \\
%                      & 0.4  & 0.30 & 0.30 & 1   & —      & —         \\
%                      & 0.5  & 0.25 & 0.25 & 1   & —      & —         \\
%                      & 0.6  & 0.20 & 0.20 & 1   & —      & —         \\
%                      & 0.7  & 0.15 & 0.15 & 1   & —      & —         \\
%                      & 0.8  & 0.10 & 0.10 & 1   & —      & —         \\
%                      & 0.9  & 0.05 & 0.05 & 1   & —      & —         \\
% \midrule
% \textbf{PLD(Ours)}                  & —    & —    & —    & 0.5 & 75.866 & 0.750461  \\
%                      & —    & —    & —    & 1.0 & \textbf{77.148} & 0.579530  \\
%                      & —    & —    & —    & 1.5 & 76.982 & 0.549435  \\
%                      & —    & —    & —    & 2.0 & 76.398 & 0.535952  \\
%                      & —    & —    & —    & 4.0 & 75.200 & 0.525917  \\
% \midrule
% PLD–ListMLE          & —    & —    & —    & $1/C$ & 74.136 & 0.532132 \\
% PLD–pListMLE         & —    & —    & —    & 1.0    & 76.588 & 0.578517 \\
% \bottomrule
% \end{tabular}
% \caption{Top‐1 accuracy and final KL (teacher→student) for all methods and hyperparameter sweeps. 
% “–” indicates not applicable. 
% \textbf{CE:} standard cross‐entropy. 
% \textbf{KD:} vanilla distillation with cross‐entropy weight $\alpha$, and temperature $\tau=2$. 
% \textbf{DIST:} relational distillation with inter‐class weight $\beta$, intra‐class weight $\gamma$, and $\tau=1$. 
% \textbf{PLD:} Plackett–Luce Distillation, sweeping $\tau$. 
% \textbf{PLD–ListMLE / PLD–pListMLE:} special cases with $\alpha_k=1/C$ and $\alpha_k=q^T_{\pi^*_k}$, respectively.}
% \label{tab:final-results}
% \end{table}



\begin{table}[ht]
\centering
\small
\caption{Top‐1 and Top‐5 accuracy for baseline methods (ResNet-50 student, ResNet-152 teacher with Top-1 Acc.\,79.61\%). “–” indicates not applicable. \textbf{CE:} standard cross‐entropy.
\textbf{LS:}\cite{szegedy2016rethinking} cross‐entropy with label smoothing ($\epsilon=0.1$). 
\textbf{KD:} vanilla distillation with mixing weight $\alpha$ and temperature $\tau=2$.
\textbf{DIST:} relational distillation with inter-class weight $\beta$, intra-class weight $\gamma$, and temperature $\tau=1$.}
\label{tab:baseline-ablation}
\begin{tabular}{lccccc c}
\toprule
\textbf{Method} & $\alpha$ & $\beta$ & $\gamma$ & $\tau$ & \textbf{Top-1 Acc.\%} & \textbf{Top-5 Acc.\%} \\
\midrule
% \multicolumn{7}{l}{\textbf{Oracle Teacher}} \\
Teacher (ResNet-152) & – & – & – & – & 79.61 & – \\
\midrule
% \multicolumn{7}{l}{\textbf{Baselines}} \\
CE                    & – & – & – & – & 71.35 & – \\
LS ($\epsilon=0.1$)   & – & – & – & – & 73.92 & – \\
\midrule
% \multicolumn{7}{l}{\textbf{Vanilla KD ($\tau=2$)}} \\
KD                     & 0.00 & – & – & 2.00 & 75.92 & 92.82 \\
                       & 0.10 & – & – & 2.00 & \textbf{76.80} & 93.16 \\
                       % & 0.20 & – & – & 2.00 & 76.65 & 93.11 \\
                       % & 0.30 & – & – & 2.00 & 76.30 & 93.02 \\
                       % & 0.40 & – & – & 2.00 & 76.33 & 93.10 \\
                       % & 0.50 & – & – & 2.00 & 76.12 & 93.12 \\
                       % & 0.60 & – & – & 2.00 & 75.94 & 92.79 \\
                       % & 0.70 & – & – & 2.00 & 75.85 & 92.71 \\
                       % & 0.80 & – & – & 2.00 & 75.21 & 92.39 \\
                       % & 0.90 & – & – & 2.00 & 74.28 & 91.59 \\
\midrule
% \multicolumn{7}{l}{\textbf{DIST ($\tau=1$)}} \\
DIST                   % & 1.00 & 2.00 & 2.00 & 1.00 & 75.77 & 92.67 \\
                       & 0.00 & 0.50 & 0.50 & 1.00 & 76.47 & 93.19 \\
                       & 0.10 & 0.45 & 0.45 & 1.00 & \textbf{76.60} & 93.30 \\
                       % & 0.20 & 0.40 & 0.40 & 1.00 & 75.69 & 92.63 \\
                       % & 0.30 & 0.35 & 0.35 & 1.00 & 74.88 & 92.18 \\
                       % & 0.40 & 0.30 & 0.30 & 1.00 & 73.90 & 91.35 \\
                       % & 0.50 & 0.25 & 0.25 & 1.00 & 72.94 & 90.95 \\
                       % & 0.60 & 0.20 & 0.20 & 1.00 & 72.71 & 90.58 \\
                       % & 0.70 & 0.15 & 0.15 & 1.00 & 71.85 & 90.16 \\
                       % & 0.80 & 0.10 & 0.10 & 1.00 & 71.89 & 90.16 \\
                       % & 0.90 & 0.05 & 0.05 & 1.00 & 71.40 & 89.88 \\
\bottomrule
\end{tabular}
\end{table}



% \begin{table}[ht]
% \centering
% \small
% \caption{Top-1 and Top-5 accuracy for PLD variants (ResNet-50 student, ResNet-152 teacher with Top-1 Acc.\,79.61\%). “–” indicates not applicable. \textbf{PLD:} Plackett–Luce Distillation sweeping temperature $\tau$. \textbf{PLD–ListMLE / PLD–pListMLE:} special cases with uniform $\alpha_k=1/C$ and data-driven $\alpha_k=q^T_{\pi^*_k}$, respectively.}
% \label{tab:pld-sweeps}
% \begin{tabular}{lccccc c}
% \toprule
% \textbf{Variant} & $\alpha$ & $\beta$ & $\gamma$ & $\tau$ & \textbf{Top-1 Acc.\%} & \textbf{Top-5 Acc.\%} \\
% \midrule
% \multicolumn{7}{l}{\textbf{Oracle Teacher}} \\
% Teacher (ResNet-152) & – & – & – & – & 79.61 & – \\
% \midrule
% \multicolumn{7}{l}{\textbf{PLD (Ours)}} \\
% PLD                     & –    & –    & –    & 0.50 & 76.06 & 92.39 \\
%                         & –    & –    & –    & 1.00 & \textbf{77.30} & 93.28 \\
%                         & –    & –    & –    & 1.50 & 77.17 & 92.74 \\
%                         & –    & –    & –    & 2.00 & 76.46 & 92.34 \\
%                         & –    & –    & –    & 4.00 & 75.22 & 91.34 \\
% \midrule
% PLD–ListMLE             & – & – & – & – & 74.11 & 90.60 \\
% PLD–pListMLE            & – & – & – & – & 76.60 & 93.23 \\
% \bottomrule
% \end{tabular}
% \end{table}


\begin{table}[ht]
\centering
\small
\caption{Top‐1 and Top‐5 accuracy for PLD variants (ResNet‐50 student, ResNet‐152 teacher with Top‐1 Acc.\,79.61\%). “–” indicates not applicable.}
% \textbf{PLD:} Plackett–Luce Distillation sweeping temperature \(\tau\). \textbf{PLD–ListMLE / PLD–pListMLE:} special cases with uniform \(\alpha_k=1/C\) and data‐driven \(\alpha_k=q^T_{\pi^*_k}\), respectively.}
\label{tab:pld-sweeps}
\begin{tabular}{l c c c}
\toprule
\textbf{Variant} & \(\tau\) & \textbf{Top-1 Acc.\%} & \textbf{Top-5 Acc.\%} \\
% \midrule
% \multicolumn{4}{l}{\textbf{Oracle Teacher}} \\
% Teacher (ResNet-152) & –    & 79.61 & –    \\
\midrule
% \multicolumn{4}{l}{\textbf{PLD (Ours)}} \\
PLD                  & 0.50 & 76.06 & 92.39 \\
                     & 1.00 & \textbf{77.30} & 93.28 \\
                     & 1.50 & 77.17 & 92.74 \\
                     & 2.00 & 76.46 & 92.34 \\
                     & 4.00 & 75.22 & 91.34 \\
\midrule
PLD–ListMLE          & –    & 74.11 & 90.60 \\
PLD–pListMLE         & –    & 76.60 & 93.23 \\
\bottomrule
\end{tabular}
\end{table}




==> sections/tables/extend.tex <==

% \begin{table}[t]
% \centering
% \small
% \caption{Top‐1 accuracy (\%) of ResNet‐50 (25.56 M) distilled on pretrained models. “Teacher Acc” is the teacher’s standalone Top‐1; KD, DIST, PLD, and Δ values are pending experiments.}
% \label{tab:pretrain-distill}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{} l r r r r r r r @{}}
% \toprule
% \multicolumn{2}{c}{} 
%   & \multicolumn{6}{c}{Top-1 \% Accuracy} \\
% \cmidrule(lr){3-8}
% Teacher (setup)       & \shortstack{Params\\(M)}
%                        & \shortstack{Teacher Acc\\(\%)} 
%                        & KD   & DIST & PLD 
%                        & \(\Delta_{\mathrm{DIST}}\) 
%                        & \(\Delta_{\mathrm{KD}}\) \\
% \midrule
% ResNet-50 (self-distill) 
%                        & 25.56   & 76.13  & – & – & – & – & – \\
% ResNet-152 (cross-arch) 
%                        & 60.19   & 78.31  & – & – & – & – & – \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

% \begin{table}[ht]
% \centering
% \small
% \caption{Top-1 accuracy (\%) of the MobileNet-v4 Medium student distilled from a MobileNet-v4 Large teacher after 100 and 300 training epochs. The “\(\Delta\)” row shows the improvement from 100 to 300 epochs.}
% \label{tab:extended-training}
% \begin{tabular}{l c c c c c}
% \toprule
% \textbf{Epochs} 
%   & \textbf{KD} 
%   & \textbf{DIST} 
%   & \textbf{PLD} 
%   & \(\Delta_{\mathrm{DIST}}\) 
%   & \(\Delta_{\mathrm{KD}}\) \\
% \midrule
% 100\,epochs 
%   & 74.86 
%   & 75.40 
%   & \textbf{75.72} 
%   & 0.32 
%   & 0.86 \\
% 300\,epochs 
%   & 76.14 
%   & 76.56 
%   & \textbf{76.94} 
%   & 0.38 
%   & 0.80 \\
% \midrule
% \(\Delta\) (300–100) 
%   & 1.28 
%   & 1.16 
%   & 1.22
%   & - 
%   & - \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[ht]
\centering
\small
\caption{Top-1 accuracy (\%) of the MobileNet-v4 Medium student distilled from a MobileNet-v4 Large teacher after 100 and 300 training epochs. The “\(\Delta\)” row shows the improvement from 100 to 300 epochs.}
\label{tab:extended-training}
\begin{tabular}{l c c c c c c}
\toprule
\textbf{Epochs} 
  & \textbf{CE} 
  & \textbf{KD} 
  & \textbf{DIST} 
  & \textbf{PLD} 
  & \(\Delta_{\mathrm{DIST}}\) 
  & \(\Delta_{\mathrm{KD}}\) \\
\midrule
100\,epochs 
  & 72.37 
  & 74.86 
  & 75.40 
  & \textbf{75.72} 
  & 0.32 
  & 0.86 \\

300\,epochs 
  & 73.04 
  & 76.14 
  & 76.56 
  & \textbf{76.94} 
  & 0.38 
  & 0.80 \\

\midrule
\(\Delta\) (300–100) 
  & 0.67 
  & 1.28 
  & 1.16 
  & 1.22 
  & – 
  & – \\
\bottomrule
\end{tabular}
\end{table}


